Local Behavior of Sparse Analysis Regularization: Applications to Risk Estimation

In this paper, we aim at recovering an unknown signal x0 from noisy L1measurements y=Phi*x0+w, where Phi is an ill-conditioned or singular linear operator and w accounts for some noise. To regularize such an ill-posed inverse problem, we impose an analysis sparsity prior. More precisely, the recovery is cast as a convex optimization program where the objective is the sum of a quadratic data fidelity term and a regularization term formed of the L1-norm of the correlations between the sought after signal and atoms in a given (generally overcomplete) dictionary. The L1-sparsity analysis prior is weighted by a regularization parameter lambda>0. In this paper, we prove that any minimizers of this problem is a piecewise-affine function of the observations y and the regularization parameter lambda. As a byproduct, we exploit these properties to get an objectively guided choice of lambda. In particular, we develop an extension of the Generalized Stein Unbiased Risk Estimator (GSURE) and show that it is an unbiased and reliable estimator of an appropriately defined risk. The latter encompasses special cases such as the prediction risk, the projection risk and the estimation risk. We apply these risk estimators to the special case of L1-sparsity analysis regularization. We also discuss implementation issues and propose fast algorithms to solve the L1 analysis minimization problem and to compute the associated GSURE. We finally illustrate the applicability of our framework to parameter(s) selection on several imaging problems.

==> aintegrer.tex <==
%This result is known to hold in the special case of synthesis regularization ($D=\Id$).
%It is proved in the overdetermined case in \cite{zou2007degrees} and is extended to the general case in~\cite{kachour2011spars}.
%In the overdetermined case with an analysis regularization, \cite{tibshirani2011solution} also proved a similar expression but with a completely different $\Hh_{\cdot,\lambda}$.
%Our expression handles both over- and underdetermined measurements with a sharper characterization of the set $\Hh_{\cdot,\lambda}$.

% The concept of degrees of freedom plays an important role in model validation and selection.
% For instance, Mallows' $C_p$ statistic provides an unbiased estimate of the {\it prediction} risk
% given by
% \begin{align}\label{eq:mallow}
%   C_p
%   =
%   \norm{y - \Phi \solS}^2
%   - N \si^2
%   + 2 \si^2 \DOF( x^\star) ~.
% \end{align}
% Many others model selection criteria involve $\DOF( x^\star)$,
% e.g. AIC, BIC and GCV.
% By replacing $\DOF( x^\star)$ in \eqref{eq:mallow} by its unbiased
% estimate given in Corollary \ref{cor:dof}, the SURE or the modified $C_p$
% statistic is still unbiased as an estimate of the {\it prediction} risk.
% We will prove this claim in the next section and extend the result to other
% risk estimators, namely the {\it projected} risk and the {\it estimation}
% risk.

% Intro
% * Dans le paragraphe de 1.4 sur le DOF il faut définir de quel risque on parle, R=E(|Phi (x^*-x0)|^2), vu qu'en plus il y en a plusieurs. Peut être ajouter que E(c_p)=R mais que c_p n'est pas calculable car DOF ne l'est pas et qu'on veut un estimateur de DOF donc de C_p.
% * "SURE can be applied to provide an estimate of the prediction risk" -> ça aura été dit clairement avant.

